Gaussian Process Optimization in the Bandit Setting: No Regret and Experimental Design

Many applications require optimizing an unknown, noisy function that is expensive to evaluate. We formalize this task as a multi-armed bandit problem, where the payoff function is either sampled from a Gaussian process (GP) or has low RKHS norm. We resolve the important open problem of deriving regret bounds for this setting, which imply novel convergence rates for GP optimization. We analyze GP-UCB, an intuitive upper-confidence based algorithm, and bound its cumulative regret in terms of maximal information gain, establishing a novel connection between GP optimization and experimental design. Moreover, by bounding the latter in terms of operator spectra, we obtain explicit sublinear regret bounds for many commonly used covariance functions. In some important cases, our bounds have surprisingly weak dependence on the dimensionality. In our experiments on real sensor data, GP-UCB compares favorably with other heuristical GP optimization approaches.

==> gp_bandit_icml_conclusions.tex <==
\vspace{-2mm}\section{Conclusions}\vspace{-1mm}

We prove the first sublinear regret bounds for GP optimization with commonly
used kernels (see \figref{regrettable}), both for $f$ sampled from a known GP
and $f$ of low RKHS norm. We analyze \ucb, an intuitive, Bayesian upper confidence bound based sampling rule.  Our regret bounds crucially depend on the information gain due to sampling, establishing a novel connection between bandit optimization and experimental design. We bound the information gain in terms
of the kernel spectrum, providing a general methodology for obtaining regret
bounds with kernels of interest.
Our experiments on real sensor network data indicate that \ucb performs at
least on par with competing criteria for GP optimization, for which no regret
bounds are known at present. Our results provide an interesting step towards
understanding exploration--exploitation tradeoffs with complex utility
functions.

%
%Our bounds suggest that the regret incurred by \ucb depends on the maximum information gain due to sampling, forging a novel connection between bandit optimization and experimental design. Our results apply both when the function $f$ is sampled from a known GP (under mild regularity conditions), or, alternatively, if $f$ is an arbitrary function with low RKHS norm $||f||_{k}$ w.r.t.~the kernel $k$ used by the algorithm. We furthermore prove bounds on the information gain, establishing sublinear regret bounds for common classes of kernel functions. Surprisingly,  for the squared exponential kernel in \emph{any} dimension, the regret grows only as $\mathcal{O}^*(\sqrt{T})$ -- the dimension $d$ appears only as exponent to a term logarithmic in $T$. 
%
